Mind the Gap! Injecting Commonsense Knowledge for Abstractive Dialogue Summarization

In this paper, we propose to leverage the unique characteristics of dialogues sharing commonsense knowledge across participants, to resolve the difficulties in summarizing them. We present SICK, a framework that uses commonsense inferences as additional context. Compared to previous work that solely relies on the input dialogue, SICK uses an external knowledge model to generate a rich set of commonsense inferences and selects the most probable one with a similarity-based selection method. Built upon SICK, SICK++ utilizes commonsense as supervision, where the task of generating commonsense inferences is added upon summarizing the dialogue in a multi-task learning setting. Experimental results show that with injected commonsense knowledge, our framework generates more informative and consistent summaries than existing methods.

==> figure_latex/error.tex <==
\begin{table}[t!]
\begin{center}\small
{\begin{tabular}{l cc cc}
    \toprule
    & \multicolumn{2}{c}{SAMSum} & \multicolumn{2}{c}{DialogSum} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5}
    & BART-xsum & SICK++ & BART-xsum & SICK++ \\
    \midrule
    % table3에서 informativeness는 바람직한 결과가 나왔는데, missing information 부분은 설문할때 세부적인 내용이 하나라도 빠지면 모두 체크한 것 같아서 좋지 않게 나왔습니다..!
    % (e.g., apples, mangos, onions, and green beans를 fruits and vegetables로 요약했으면 missing information으로 체크해버림)
    % error analysis에서 missing information을 빼는건 어떨까요..?
    % informativeness와 상충될 우려가 있는 것 같습니다.
    (i) & 25.34 & 24.67 & 29.34 & 31.34 \\
    (ii) & 27.33 & 20.00 & 24.67 & 24.67 \\
    (iii) & 10.00 & 8.00 & 6.67 & 3.37 \\
    (iv) & 7.33 & 2.00 & 13.34 & 1.33 \\
    \bottomrule
\end{tabular}}
\end{center}
\caption{Results of error analysis where each value denotes the number of generated summaries belongs to the corresponding error type.}
\label{tab:error}
\end{table}



\begin{comment}
\begin{table}[t!]
\begin{center}\small
{\begin{tabular}{l cc}
    \toprule
    Error Type & SAMSum & DialogSum \\
    \midrule
    Missing information \\ 
    Wrong references \\
    Improper reasoning \\ 
    Incorrect name \\
    \bottomrule
\end{tabular}}
\end{center}
\caption{Results of error analysis where each value denotes the number/percentage of generated summaries belongs to the corresponding error type.}
\label{tab:error}
\end{table}
\end{comment}

==> figure_latex/relation_similarity.tex <==
\begin{table}[t!]
\begin{center}\small
{\begin{tabular}{ll r}
    \toprule
    & Relation & Similarity \\
    \midrule
    \multirow{7}{*}{\begin{sideways}Physical-Entity\end{sideways}}
    & \textsc{ObjectUse} & 0.219281 \\
    & \textsc{AtLocation} & 0.188235 \\
    & \textsc{MadeUpOf} & 0.228884 \\
    & \textsc{HasProperty} & 0.205886 \\
    & \textsc{CapableOf} & 0.198517 \\
    & \textsc{Desires} & 0.196573 \\
    & \textsc{NotDesires} & 0.237048 \\
    \midrule
    \multirow{7}{*}{\begin{sideways}Event-Centered\end{sideways}}
    & \textsc{isAfter} & 0.287347 \\
    & \textsc{HasSubEvent} & 0.195233 \\
    & \textsc{isBefore} & 0.293669 \\
    & \textsc{HinderedBy} & 0.330957 \\
    & \textsc{Causes} & 0.261371 \\
    & \textsc{xReason} & 0.293779 \\
    & \textsc{isFilledBy} & 0.158177 \\
    \midrule
    \multirow{9}{*}{\begin{sideways}Social-Interaction\end{sideways}}
    & \textsc{xNeed} & 0.226811 \\   
    & \textsc{xAttr} & 0.155394 \\
    & \textsc{xEffect} & 0.178730 \\
    & \textsc{xReact} & 0.134452 \\
    & \textsc{xWant} & 0.232237 \\
    & \textsc{xIntent} & 0.200213 \\
    & \textsc{oEffect} & 0.182719 \\
    & \textsc{oReact} & 0.120556 \\
    & \textsc{oWant} & 0.205300 \\
    \bottomrule
\end{tabular}
}
\end{center}
\caption{The similarity scores broken down by the relation types of COMET.}
\label{tab:relation_siimilarity_comet}
\end{table}



\begin{table}[t!]
\begin{center}\small
{\begin{tabular}{ll r}
    \toprule
    & Relation & Similarity \\
    \midrule
    \multirow{3}{*}{\begin{sideways}Causes\end{sideways}}
    & \textsc{xIntent} & 0.188765 \\
    & \textsc{xNeed} & 0.206658\\
    & \textsc{xAttr}& 0.121815 \\
    \midrule
    \multirow{6}{*}{\begin{sideways}Effects\end{sideways}}
    & \textsc{xWant}  & 0.186658 \\
    & \textsc{xEffect}& 0.208305\\
    & \textsc{xReact} & 0.099631 \\
    & \textsc{oWant}& 0.181103\\
    & \textsc{oEffect}& 0.147515\\
    & \textsc{oReact}& 0.099683\\
    \bottomrule
\end{tabular}
}
\end{center}
\caption{The similarity scores broken down by the relation types of PARA-COMET.}
\label{tab:relation_siimilarity_paracomet}
\end{table}




\begin{comment}

    & CausesDesire& 0.255257 \\
    & CreatedBy& 0.211708 \\
    & DefinedAs& 0.265975 \\
    & DesireOf& 0.242964802548495 \\

    & HasA & 0.2451534110216064 \\


    & HasFirstSubevent& 0.23733915450146528 \\
    & HasLastSubevent& 0.2716753018140833 \\
    & HasPainCharacter& 0.26636885634273305 \\
    & HasPainIntensity & 0.22521264288591697 \\
    & HasPrerequisite & 0.22930974846820656 \\


    & HasSubevent& 0.2237412262715584 \\ 
 
    & InheritsFrom& 0.23259012133268656 \\
    & InstanceOf & 0.23212968720216745 \\
    & IsA& 0.2561858685648585 \\
    & LocatedNear& 0.21253568460701902 \\
    & LocationOfAction& 0.2135756227519609 \\
    & MadeOf& 0.25319490144326257 \\

    & MotivatedByGoal  &   0.2628675263826433 \\
    & NotCapableOf &  0.23558798329718475\\

    & NotHasA& 0.29718137531390604\\
    & NotHasProperty & 0.18850054675998132\\
    & NotIsA& 0.2682374839010364\\
    & NotMadeOf& 0.2646789299019957\\
    

    & PartOf& 0.2340617114107215\\
    & ReceivesAction& 0.2347766847998503\\
    & RelatedTo& 0.24442570201676214\\
    & SymbolOf& 0.24776872832778457\\
    & UsedFor& 0.22900067080225753\\
\end{comment}
